Solving High Frequency and Multi-Scale PDEs with Gaussian Processes

Machine learning based solvers have garnered much attention in physical simulation and scientific computing, with a prominent example, physics-informed neural networks (PINNs). However, PINNs often struggle to solve high-frequency and multi-scale PDEs, which can be due to spectral bias during neural network training. To address this problem, we resort to the Gaussian process (GP) framework. To flexibly capture the dominant frequencies, we model the power spectrum of the PDE solution with a student $t$ mixture or Gaussian mixture. We apply the inverse Fourier transform to obtain the covariance function (by Wiener-Khinchin theorem). The covariance derived from the Gaussian mixture spectrum corresponds to the known spectral mixture kernel. Next, we estimate the mixture weights in the log domain, which we show is equivalent to placing a Jeffreys prior. It automatically induces sparsity, prunes excessive frequencies, and adjusts the remaining toward the ground truth. Third, to enable efficient and scalable computation on massive collocation points, which are critical to capture high frequencies, we place the collocation points on a grid, and multiply our covariance function at each input dimension. We use the GP conditional mean to predict the solution and its derivatives so as to fit the boundary condition and the equation itself. As a result, we can derive a Kronecker product structure in the covariance matrix. We use Kronecker product properties and multilinear algebra to promote computational efficiency and scalability, without low-rank approximations. We show the advantage of our method in systematic experiments. The code is released at \url{https://github.com/xuangu-fang/Gaussian-Process-Slover-for-High-Freq-PDE}.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\cmt{
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
	justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
	\item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
}


\begin{enumerate}
	
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{}
		\item Did you describe the limitations of your work?
		\answerYes{}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNA{}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerNA{}
		\item Did you include complete proofs of all theoretical results?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerYes{}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerYes{}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerYes{}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerYes{}
		\item Did you mention the license of the assets?
		\answerNA{}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNA{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{}
	\end{enumerate}
	
	
\end{enumerate}

==> exp-fang.tex <==
\section{Experiment}\label{section:exp}
To evaluate \ours, we considered three commonly-used benchmark PDE families in the literature of machine learning solvers~\citep{raissi2019physics,wang2021eigenvector,krishnapriyan2021characterizing}. Following the prior works, we fabricated a series of solutions to thoroughly examine the performance. 

\noindent\textbf{The Poisson Equation}. We first considered 1D and 2D Poisson equations with different source functions that lead to various scale information in the solution. We used Dirichlet boundary conditions. 
\begin{align}
	u_{xx} &= f(x), \;\; x \in [0, 2\pi], \notag \\
	u_{xx} + u_{yy} &= f(x, y), \;\; (x, y) \in [0, 2\pi] \times [0, 2\pi].
\end{align}
For the 1D Poisson equation, we created source functions $f$ that give the following high-frequency and multi-frequency solutions, $u_1 = \sin(100x)$, $u_2 = \sin(x) + 0.1\sin(20x) + 0.05\cos(100x)$, $u_3 = \sin(6x)\cos(100x)$, and $u_4 = x \sin(200x)$. In addition, we tested with a \textit{challenging} hybrid solution that mixes a high-frequency with a quadratic function,  $u_5 = \sin(500x) - 2(x - 0.5)^2$ where we set $x \in [0, 1]$. For the 2D Poisson equation, we tested with the following multi-scale solutions, $u_6 = \sin(100x)\sin(100 y)$ and $u_7 = \sin(6x) \sin(20x) + \sin(6 y) \sin(20y)$. 

\noindent\textbf{Allen-Cahn Equation}. We next considered 1D and 2D Allen-Cahn (nonlinear diffusion-reaction) equations with different source functions and Dirichlet boundary conditions. %Note that these are nonlinear equations.
\begin{align}
	u_{xx} + u(u^2 - 1) &= f(x), \;\; x \in [0, 2\pi], \notag \\
	u_{xx} + u_{yy} + u(u^2 - 1) &= f(x, y), \;\; (x,y) \in[0, 1] \times [0, 1]. \label{eq:allen-cahn}
\end{align}
For the 1D equation, we tested with solutions $u_1 = \sin(100x)$ and $u_2 = \sin(6x)\cos(100x)$. For the 2D equation, we created the source $f$ that gives the following mixed-scale solution, $u = \left(\sin(x) + 0.1\sin(20x) + \cos(100x)\right) \cdot \left(\sin(y) + 0.1\sin(20y) + \cos(100y)\right).$

\noindent\textbf{Advection Equation.} Third, we evaluated with a 1D advection (one-way) equation, 
\begin{align}
	u_t + 200 u_x  = 0, \;\;\; x \in [0, 2\pi], \;\;t \in [0, 1].
\end{align}
We used the Dirichlet boundary conditions, and the solution has an analytical form, $u(x, t) = h(x - 200t)$ where $h(x)$ is the initial condition for which we chose as $h(x) = \sin(x)$.


We compared with the following state-of-the-art ML solvers: (1) standard PINN, (2) Weighted PINN (W-PINN) that up-weight the boundary loss to reduce the dominance of the residual loss, and to more effectively propagate the boundary information,  (3) Rowdy~\citep{jagtap2022deep}, PINN with an adaptive activation function, which combines a standard activation with several $\sin$ or $\cos$ activations. (4) RFF-PINN, feeding Random Fourier Features to the  PINN~\citep{wang2021eigenvector}. To ensure RFF-PINN achieves the best performance, we followed~\citep{wang2020and} to dynamically re-weight the loss terms based on NTK eigenvalues~\citep{wang2020and}.  (5) Spectral Method~\citep{boyd2001chebyshev}, which approximations the solution with a linear combination of trigonometric bases, and estimates the basis coefficients via least mean squares.  In addition, we also tested (6) GP-SE and (7) GP-Mat\'ern,  GP solvers with the square exponential (SE)  and the Mat\'ern kernel. We also test traditional solvers: (8) Chebfun\footnote{\url{https://www.chebfun.org/}} that solves PDEs based on Chebyshev interpolants, (9) Finite Difference (FD), which solves the PDEs via discretization based on finite difference. We denote our method using the covariance function based on \eqref{eq:smm} and \eqref{eq:sm} by \ours-StM and \ours-GM, respectively. The details about the hyperparameter setting and baselines implement are provided in Section~\ref{sect:expr-setting} of Appendix. 



\begin{table*}[t]
	%\begin{wraptable}{r}{0.7\textwidth}
	\vspace{-0.01in}
	\small
	\centering
	%\begin{subtable}{\textwidth}
	%\centering
	\begin{tabular}[c]{cccccccc}
		\toprule
		\multirow{2}{*}{\textit{Method}} & \multicolumn{5}{c}{1D} & \multicolumn{2}{c}{2D}\\
		\cline{2-8}
		& $u_1$  & $u_2$ & $u_3$ & $u_4$  & $u_5$ & $u_6$ & $u_7$\\
		\hline 
		PINN 			& $1.36e{0}$ & $1.40e{0}$ & $1.00e{0}$ &  $1.42e{1}$ & $6.03e{-1}$ & $1.63e{0}$ & $9.99e{-1}$\\
		W-PINN 			& $1.31e{0}$ & $2.65e{-1}$ & $1.86e{0}$ & $2.60e{1}$ & $6.94e{-1}$ &  $1.63e{0}$& $6.75e{-1}$\\
		RFF-PINN 		& $4.97  e{-4}$  & ${2.00 e{-5}}$ & $7.29 e{-2}$ & $2.80 e{-1}$ & $5.74 e{-1}$ &  $1.69 e{0}$ & $7.99  e{-1}$\\
		Rowdy 			& $1.70 e{0}$ & $1.00e{0}$ & $1.00e{0}$ & $1.01e{0}$ & $1.03e{0}$   & $2.24e{1}$ & $7.36e{-1}$\\
		{Spectral method} & {$2.36 e{-2}$} & {$3.47e{0}$} & {$1.02e{0}$} & {$1.02e{0}$} & {$9.98e{-1}$} &  {$1.58e{-2}$} & {$1.04 e{0}$}\\
		% {Chebfun} &{3.05e-11} &{1.17e-11} & {5.81e-11} & {1.14e-10} &{8.95e-10} & {N/A} & {N/A} \\
		{Chebfun} &${3.05e-11}$ &${1.17e-11}$ & ${5.81e-11}$ & ${1.14e-10}$ &${8.95e-10}$ & {N/A} & {N/A} \\

		{Finite Difference} & {5.58e-1} & {4.78e-2} & {2.34e-1} & {1.47e0 } & {1.40e0} & {2.33e-1} & {1.75e-2} \\  
		\hline
		GP-SE          &  $2.70 e{-2}$& $9.99 e{-1}$ &$9.99 e{-1}$  & $3.19 e{-1}$	& $9.75 e{-1}$ & $9.99 e{-1}$ &$9.53 e{-1}$\\
		GP-Mat\'ern  & $3.32 e{-2}$ & $9.8 e{-1}$  &$5.15 e{-1}$  & $1.83 e{-2}$	& $6.27 e{-1}$  	&$6.28 e{-1}$		& $3.54 e{-2}$\\
		\ours-GM     & $\bold{3.99 e{-7}}$ & $2.73 e{-3}$ 	 & $3.92 e{-6}$ & $1.55 e{-6}$   & $1.82 e{-3}$	   &  	$\bold{6.46 e{-5}}$ & $1.06 e{-3}$\\
		\ours-StM  & $6.53 e{-7}$ & $\bold{2.71 e{-3}}$&$\bold{3.17 e{-6}}$  & $\bold{8.97 e{-7}}$ & $\bold{4.22 e{-4}}$  & $6.87 e{-5}$ & $\bold{1.02 e{-3}}$\\
		\bottomrule
	\end{tabular}
	% \caption{\small 10 data points.}
	%  \end{subtable}
	%\vspace{-0.05in}
	\caption{\small  Relative $L_2$ error in solving 1D and 2D Poisson equations, where $u_j$'s are different high-frequency and multi-scale solutions:  $u_1 = \sin(100x)$, $u_2 = \sin(x) + 0.1\sin(20x) + 0.05\cos(100x)$, $u_3 = \sin(6x)\cos(100x)$,  $u_4 = x \sin(200x)$, $u_5 = \sin(500x) - 2(x - 0.5)^2$,  $u_6 = \sin(100x)\sin(100 y)$ and $u_7 = \sin(6x) \sin(20x) + \sin(6 y) \sin(20y)$. } \label{tb:1d-poisson}
%	\vspace{-0.2in}
\end{table*}
\begin{table*}[h]
	%\begin{wraptable}{r}{0.7\textwidth}
	\vspace{-0.01in}
	\small
	\centering
	%\begin{subtable}{\textwidth}
	%\centering
	\begin{tabular}[c]{ccccc}
		\toprule
		\multirow{2}{*}{\textit{Method}} & \multicolumn{2}{c}{1D Allen-cahn } & \multirow{2}{*}{2D Allen-cahn} & \multirow{2}{*}{1D Advection} \\
		\cline{2-3}
		& $u_1$  & $u_2$ &  & \\
		\hline 
		PINN & $1.41 e{0}$ & $1.14 e{1}$ & $1.96 e{1}$ & $1.00 e{0}$ \\
		W-PINN & $1.34 e{0}$ & $1.45 e{1}$ & $2.03 e{1}$ & $1.01 e{0}$ \\
		RFF-PINN & $1.24 e{-3}$ & $2.46 e{-1}$ & $7.17 e{-1}$ & $9.96 e{-1}$ \\
		Rowdy & $1.30 e{0}$ & $1.31 e{0}$ & $1.18 e{0}$ & $1.03 e{0}$ \\
		{Spectral method}& {$2.34 e{-2}$} & {$2.45 e{1}$} & {$2.45 e{1}$} & {$2.67 e{0}$}\\
		{Chebfun} & {1.39e-08} & {2.94e-10} & {N/A} & {1.39e0}\\
		{Finite Difference} & {2.32e-01} & {2.36e-1} & {3.23e0} & {1.29e-1}\\ 
		\hline
		GP-SE  &  $2.74 e{-2}$   	& $1.06 e{-2}$    & $3.48 e{-1}$ & $9.99 e{-1}$ \\
		GP-Mat\'ern  & $3.32 e{-2}$ 	& $5.16 e{-2}$   & $2.96 e{-1}$ & $9.99 e{-1}$ \\
		\ours-StM  & $7.71 e{-6}$	 & $4.76 e{-6}$ & $\bold{2.99 e{-3}}$ & $\bold{9.08 e{-4}}$ \\
		\ours-GM  & $\bold{4.91 e{-6}}$	&  $\bold{4.24 e{-6}}$&$5.78 e{-3}$ & $3.59 e{-3}$ \\
		\bottomrule
	\end{tabular}
	% \caption{\small 10 data points.}
	%  \end{subtable}
	%\vspace{-0.05in}
	\caption{\small Relative $L_2$ error in solving 1D, 2D Allen-cahn equations and 1D advection equation, where $u_1$ and $u_2$ are two test solutions for 1D Allen-cahn: $u_1 = \sin(100x)$, $u_2 = \sin(6x)\cos(100x)$. The test solution for 2D Allen-cahn is $\left(\sin(x) + 0.1\sin(20x) + \cos(100x)\right) \cdot  \left(\sin(y) + 0.1\sin(20y) + \cos(100y)\right)$, and for 1D advection equation is $\sin(x-200t)$.  } \label{tb:allen}
	\vspace{-0.2in}
\end{table*}

% add figures
\noindent\textbf{Solution Accuracy.} We report the relative $L_2$ error (normalized root-mean-square error) of each method in Table \ref{tb:1d-poisson} and \ref{tb:allen}.  The best result and the smaller error between \ours-StM and \ours-GM are made bold. We can see that our method achieves the smallest solution error among most cases compared with PINN-based methods. In all the cases, the solution error of \ours achieves at least 1e-3 level. In quite a few cases, our method even reaches an error around 1e-6 and 1e-7. It shows  that \ours  can successfully solve all these equations.\cmt{ and accurately capture the high-frequency and multi-scale information.} GP solvers using the plain SE and Mat\'ern kernel result in several orders of the magnitude bigger errors. The standard PINN and W-PINN basically failed to solve every equation. While Rowdy improved upon PINN and W-PINN in most cases, the error is still quite large. The inferior performance of the spectral method implies that only using trigonometric bases is not sufficient. With the usage of the random Fourier features,  RFF-PINN can greatly boost the performance of PINN and W-PINN in many cases. %However, it still failed in many cases.
 {However, in the most cases, it is still much inferior to \ours.}  {Compared with traditional solvers, we can see Chebfun performs very well, and achieves the highest solution accuracy except for the 1D advection problem. However, Chebfun is limited to 1D problems and temporal PDEs. It cannot handle 2D stationary PDEs, no matter linear or nonlinear.  Finite Difference can provide reasonable accuracy, but the performance is consistently much worse than \ours.  Overall, we can see that our method is general enough to solve different types of PDEs (1D/2D, linear/nonlinear, stationary and non-stationary); to achieve a satisfactory accuracy, we do NOT need to change our computation framework to re-develop the solver.}
 


\textbf{Point-wise Error.} We then show the point-wise solution error in Fig. \ref{fig:poisson1d-mix_sin},  \ref{fig:poisson1d-x2_add_sinx}, \ref{fig:allencahn-2d_error},  and in Appendix Fig. \ref{fig:poisson1d-x_time_sinx}, \ref{fig:poisson2d-sin_add_cos_error}, \ref{fig:advection_error}. We can see that GP-SE is difficult to capture high frequencies. While GP-Mat\'ern is better, it is unable to grasp all the scale information. RFF-PINN successfully captured multi-scale frequencies in Fig. \ref{fig:poisson1d-mix_sin}, but it failed in more challenging cases as in Fig.   \ref{fig:poisson1d-x2_add_sinx} and \ref{fig:allencahn-2d_error}. In 2D Poisson and 1D Advection,  the point-wise error of both \ours-StM and \ours-GM is quite uniform across the domain and is close to zero (dark blue); see Fig. \ref{fig:allencahn-2d_error}, and in Appendix Fig.  \ref{fig:poisson2d-sin_add_cos_error}, \ref{fig:advection_error}. By contrast, the other methods exhibit  large errors in a few local regions.  Together these results show that \ours not only gives a superior global accuracy, but locally recovers individual solution values.

\textbf{Frequency Learning.} Third, we investigated the learned component weights $w_q$ and frequencies $\mu_q$ of \ours. In Fig. \ref{fig:sparsity}, we show the results for two Poisson equations. As we can see, although the number of components $Q$ is set to be much more than the true frequencies, the estimation of most weights $w_q$ is very small (less than $10^{-10}$). That means, excessive frequency components have been automatically pruned. The remaining components with significant weights completely match the number of true frequencies in the solution. The frequency estimation $\mu_q$ is very close to the ground-truth. This demonstrates that the implicit Jefferys  prior (by optimizing $w_q$ in the log space) can indeed implement sparsity, select the right frequency number, and recover the ground-truth frequency values. 

\begin{figure*}[t]
	%	\vspace{-0.05in}
	\setlength{\tabcolsep}{0pt}
	\centering
	\includegraphics[width=\linewidth]{./figs_fang/poisson_1d-mix_sin/pred_sum.pdf}
	\caption{\small Prediction for  the 1D Poisson equation with solution  $\sin(x) + 0.1\sin(20x) + 0.05\cos(100x)$.}
	%\vspace{0.02in}
	\label{fig:poisson1d-mix_sin}
\end{figure*}
\begin{figure*}[t]
	%	\vspace{-0.05in}
	\setlength{\tabcolsep}{0pt}
	\centering
	\includegraphics[width=\linewidth]{./figs_fang/poisson_1d-x2_add_sinx/pred_sum.pdf}
	\caption{\small Prediction for the 1D Poisson equation with solution $\sin(500x)-2(x-0.5)^2$.}
	%	\vspace{0.02in}
	\label{fig:poisson1d-x2_add_sinx}
\end{figure*}
\begin{figure*}[h!]
	%	\vspace{-0.05in}
	\setlength{\tabcolsep}{0pt}
	\centering
	\includegraphics[width=\linewidth]{./figs_fang/allencahn_2d-mix-sincos/error_sum.pdf}
	\caption{\small  Point-wise solution error for 2D Allen-cahn equation, and the solution is $\left(\sin(x) + 0.1\sin(20x) + \cos(100x)\right)  \left(\sin(y) + 0.1\sin(20y) + \cos(100y)\right)$.}
	%	\vspace{0.02in}
	\label{fig:allencahn-2d_error}
\end{figure*}


\begin{figure*}[h!]
	%	\vspace{-0.05in}
	\centering
	\setlength{\tabcolsep}{0pt}
	\begin{tabular}[c]{ccc}
		\begin{subfigure}[b]{0.33\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs_fang/sparsity/freq_weight_poisson_1d_sincos.pdf}
			\caption{\small Poisson-1D}
			\label{fig:sparsity-poisson_1d-sin_cos}
		\end{subfigure} &
		\begin{subfigure}[b]{0.315\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs_fang/sparsity/freq_weight_1_poisson_2d_sin_sin-x.pdf}
			\caption{\small  Poisson-2D $x$-dim}
			\label{fig:sparsity-poisson_2d-sin_sin-x}
		\end{subfigure} &
		\begin{subfigure}[b]{0.32\textwidth}
			\centering
			\centering
			\includegraphics[width=\linewidth]{./figs_fang/sparsity/freq_weight_1_poisson_2d_sin_sin-y.pdf}
			\caption{\small Poisson-2D $y$-dim}
			\label{fig:sparsity-poisson_2d-sin_sin-y}
		\end{subfigure}
	\end{tabular}
	%\vspace{-0.1in}
	\caption{\small The learned component weights and frequency values. For each number pair a(b) in the figure, ``a'' is the learned frequency by \ours, and ``b'' is the ground-truth. The expressions on the top are the solutions.  }
	\vspace{-0.2in}
	\label{fig:sparsity}
\end{figure*}
%\setlength{\columnsep}{10pt}
%\begin{wrapfigure}[h!]
%\begin{wrapfigure}{r}{0.6\textwidth}

\textbf{Influence of Collocation Point Quantity}. Fourth, we examined how the number of collocation points influences the solution accuracy. To this end, we tested with a 1D Poisson  and 2D Poisson equation, whose solutions include high frequencies. Due to the space limit, we leave the results and discussion in Section \ref{sect:appendix:clo-point} of Appendix. 

\textbf{Learning behavior and efficiency.} Finally, we investigated the learning behavior and computational efficiency of \ours as compared with the PINN and its variants. Due to the space limit, we leave the results and discussion in Section \ref{sect:appendix:learn} of Appendix. 




==> method-backup.tex <==
%GP priors--> different from their method, we place a GP prior over the function values at the grid, and then interpolate the values ... . The advantage is that we can use .... 
%next  
\section{Gaussian Process}
Gaussian processes (GPs) provide an expressive framework for function estimation. Suppose given a training dataset $\Dcal = \{(\x_n , y_n)| 1\le n \le N\}$,  we aim to estimate a target function $f: \mathbb{R}^d \rightarrow \mathbb{R}$. We can assign a GP prior, $$f(\cdot) \sim \gp(m(\cdot), \cov(\cdot,\cdot)),$$ where $m(\cdot)$ is the mean function and $\cov(\cdot, \cdot)$ is the covariance function. In practice, one often sets $m(\cdot) = 0$, and adopts a kernel function as the covariance function, namely $\cov\left(f(\x), f(\x')\right) = k(\x, \x')$.  For example, a popular kernel function is the square exponential (SE) kernel, $k(\x, \x') = \exp\left(- \|\x - \x'\|^2/\rho\right)$. A nice property of the GP prior is that if $f$ is sampled from a GP, then any derivative (if existent) of $f$ is also a GP, and the covariance between the derivative and the function $f$ is the derivative of the kernel function w.r.t the same input variable(s). For example, 
\begin{align}
	\cov(\partial_{x_1x_2} f(\x), f(\x')) = \partial_{x_1x_2} k(\x, \x') \label{eq:cov-der-1}
\end{align}
where $\x = (x_1, \ldots, x_d)^\top$ and $\x' = (x_1', \ldots, x_d')^\top$.  

Under the GP prior, the function values at any finite input collection, $\f = [f(\x_1), \ldots, f(\x_N)]$, follow a multi-variate Gaussian distribution, $p(\f) = \N(\f|\0, \K)$ where $[\K]_{ij} = \cov(f(\x_i), f(\x_j)) = k(\x_i, \x_j)$. Suppose given $\f$,  we want to compute the distribution of the function value at any input $\x$, namely $p(f(\x) | \f)$. Since $\f$ and $f(\x)$ also follow a multi-variate Gaussian distribution, we obtain a conditional Gaussian, $p(f(\x) | \f) = \N\left(f(\x) | \mu(\x), \sigma^2(\x)\right)$, where
\begin{align}
	\mu(\x) = \cov(f(\x), \f) \K^{-1} \f,  
\end{align}
and $\sigma^2(\x) = \cov(f(\x), f(\x)) -  \cov(f(\x), \f) \K^{-1}  \cov(\f, f(\x))$, $\cov(f(\x), \f) = k(\x, \X) = [k(\x, \x_1), \ldots, k(\x, \x_N)]$ and $\X = [\x_1, \ldots, \x_N]^\top$. We can then use a Gaussian noise model to fit the actual observations $\y = [y_1, \ldots, y_N]^\top$,  namely, $p(\y|\f) = \N(\y | \f, \tau^{-1}\I)$. % where $v$ is the noise variance.
\section{Gaussian Process PDE Solvers}
Now we present our GP solver.  When the solution $u(\x)$  includes high frequencies or multi-scale information, one naturally wants to estimate these target frequencies outright in the frequency domain. To this end, we consider the solution's power spectrum, $S(\s) = |\uhat(\s)|^2$ where $\uhat(\s) = \int u(\x)e^{-i 2\pi \s^\top \x} \d \x$ is the Fourier transform of the solution $u$. Here $i$ indicates complex numbers and $\s$ denotes the frequency.  The power spectrum characterizes the strength of every possible frequency  (\ie power) underlying the solution $u$. To flexibly capture the dominant high and/or multi-scale frequencies, we use a mixture of student $t$ distributions to model the power spectrum, 
\begin{align}
	 S(\s) = \sum\nolimits_{q=1}^Q w_q \text{St}(s; \mu_q, \rho_q^2, \nu) \label{eq:st-mix}
\end{align}
where $w_q \ge 0$ is the weight for component $q$, $\text{St}$ stands for student $t$ distribution, $\mu_q$ is the mean, $\rho_q$ is the inverse variance, and $\nu$ is the degree of freedom. Note that $w_q$ does not need to be normalized (their summation is not necessary to be one).  Each student $t$ distribution characterizes one principle frequency (\ie $\mu_q$), and it also robustly models the (potentially many) minor frequencies with a fat tailed density [\zhec{bishop}]. An alternative choice is a mixture of Gaussian, $S(\s) = \sum_{q=1}^Q w_q \N(s; \mu_q, \rho_q \I)$. However, the Gaussian distribution has thin tails in density and hence is less robust (in capturing minor frequencies). 

Next, we convert the spectrum model into the covariance space to enable our GP solver to flexibly capture the target frequencies. According to the Wiener-Khinchin theorem \zhec{ref}, for a wide-sense stationary random process, under mild conditions, its power spectrum and the auto-correlation form a Fourier pair. In our method, we model $u$ as drawn from a stationary GP, and hence the auto-correlation becomes the covariance function of the GP, denote by $k(\x, \x') = k(\x - \x')$. We then have
\begin{align}
	S(\s) = \int k(\z)e^{-i 2\pi \s^\top \z } \d\z, \;\;\; k(\z) = \int S(\s) e^{i 2\pi \z^\top \s} \d \s \label{eq:wk}
\end{align} 
where $\z = \x - \x'$. Therefore, we can obtain the covariance function by applying the inverse Fourier transform over the student $t$ or Gaussian mixture model for $S(\s)$. However,  the straightforward mixture form in  \eqref{eq:st-mix} will lead to a complex-valued covariance function after inverse Fourier transform. To obtain a real-valued covariance, inside each component we add another student $t$ distribution with mean $-u_q$ so as to cancel out the imaginary part in the integral. In addition, to make the derivation convenient, we scale the inverse variance and degree freedom parameters by some constant. We then use the following power spectrum model, 
\begin{align}
	S(s) = \sum_{q=1}^Q w_q \left(\text{St}(s; \mu_q, 4\pi^2\rho_q^2, 2\nu) +\text{St}(s; -\mu_q, 4\pi^2\rho_q^2, 2\nu) \right). \label{eq:mix2}
\end{align}
Applying inverse Fourier transform in \eqref{eq:wk}, we can derive the following covariance function, 
\begin{align}
	k_{StM}(x, x') = \sum\nolimits_{q=1}^Q w_q \gamma_{\nu, \rho_q}(x, x') \cos(2\pi \mu_q (x - x'))
\end{align} 	
where $\gamma_{\nu, \rho_q}(x, x') = \frac{2^{1-\nu}}{\Gamma(\nu)}\left(\sqrt{2\nu}\frac{|x - x'|}{\rho_q}\right)^{\nu} K_\nu(\sqrt{2\nu}\frac{|x - x'|}{\rho_q})$ is the Mat\'ern kernel with degree of freedom $\nu$ and length scale $\rho_q$, and $K_\nu$ is the modified Bessel function of the second kind.  We now can see that the frequency information $\mu_q$ and the component weights $w_q$ are embedded into the covariance function.  By learning a GP model, we expect to capture the true frequencies of the solution. One can also construct a symmetric Gaussian mixture, $S(\s) = \sum\nolimits_{q=1}^Q w_q \left(\N(\s | \bmu_q, \diag(\v_q)) + \N(\s | -\bmu_q, \diag(\v_q))\right)$. Via inverse Fourier transform, we obtain
\begin{align}
	k_{\text{GM}}(x, x') = \sum\nolimits_{q=1}^Q w_q \exp\left(-\rho_q (x - x')^2\right)\cdot  \cos(2\pi (x - x') \mu_q).
\end{align}
This is known as the spectral mixture kernel~\citep{wilson2013gaussian}, which was originally proposed to construct an expressive stationary kernel according to its Fourier decomposition, because in principle the Gaussian mixture can well approximate 
any distribution, as long as using enough many components. In~\citep{wilson2013gaussian}, the spectral mixture kernel can well recover many popular kernels, such as rational quadratic and periodic kernel. 
In this paper, we take a different viewpoint and motivation. We argue that a similar design can be very effective in extracting dominant frequencies in PDE solving. 

Since the number of dominant frequencies is unknown a priori, the solution accuracy can be sensitive to the choice of the component number $Q$. A too small $Q$ can miss important (high) frequencies while a too big $Q$ can bring in excessive noisy frequencies. To address this problem, we can set a large $Q$ (\eg $Q = 50$), and then optimize the component weights in the log domain. This is actually equivalent to assigning each $w_q$ a Jefferys prior. Specifically, define $\wbar_q = \log(w_q)$. Since we do not place an additional prior over $\wbar_q$, we can view $p(\wbar_q) \propto 1$. Then we have  
\begin{align}
	p(w_q) = p(\wbar_q) \left|\frac{\d \wbar_q}{\d w_q}\right| \propto \frac{1}{w_q}.
\end{align}
The Jefferys prior has very a high density close to zero, and it can induce the strong sparsity during the learning of $w_q$. Accordingly, the excessive frequency components can be automatically pruned, and the learning can drive the remaining frequency parameters toward the target frequencies. This is verified by our experiments. See XXX. 




Now we present our GP based PDE solver. Given the PDE of the general form \eqref{eq:pde}, we assign a GP prior over the solution, $u \sim \gp(0, k(\cdot, \cdot))$. To accurately and efficiently estimate $u$ from the boundary conditions and equation, we create a grid on the domain $\Omega$. Note that the grid is unnecessary to be evenly spaced. We can randomly sample or specially design the locations at each input dimension, and then construct the grid through a Cartesian product. Denote the locations at each input dimension $j$ by $\h_j = [h_{j1}, \ldots, h_{jM_j}]$, we have an $M_1 \times \ldots \times M_d$ grid, 
\begin{align}
	\Gcal = \h_1 \times \ldots \times \h_d = \{\x=(x_1, \ldots, x_d) | x_j \in \h_j, 1\le j \le d\}.
\end{align} 
We will use the grid points on the boundary $\partial \Omega$ to fit the boundary conditions and all the grid points as  the collocation points to fit the equation. 

Denote the solution values at $\Gcal$ by $\Ucal = \{u(\x)| \x \in \Gcal\}$, which is an $M_1 \times \ldots \times M_d$ array. According to the GP prior over $u(\cdot)$, we have a multi-variate Gaussian prior distribution over $\Ucal$, 
\begin{align}
	p(\Ucal) = \N(\vec(\Ucal)| \0, \C) \label{eq:prior-over-grid}
\end{align} 
where $\vec(\cdot)$ is to flatten $\Ucal$ into a vector, $\C$ is the covariance matrix computed from $\Gcal$ with kernel function $k(\cdot, \cdot)$. 
Denote the grid points on the boundary by $\Bcal = \Gcal \cap \partial \Omega$. To fit the boundary condition, we use a Gaussian likelihood, 
\begin{align}
	p(\g | \u_\Bcal) = \N(\g|\u_b, \tau_1^{-1}\I) \label{eq:boundary-ll}
\end{align}
where $\g = \vec\left(\{g(\x) | \x \in \Bcal\}\right)$, $\u_b$ are the values of $\Ucal$ on $\Bcal$ (that are flatten into a vector), and $\tau_1>0$ is the inverse variance. Next, we want to fit the equation at $\Gcal$. To this end, we need to first obtain the prediction of all the relevant derivatives of $u$ in the PDE, \eg $\partial_{x_1} u$ and $\partial_{x_1x_2} u$, at the grid $\Gcal$. Since $u$'s derivatives also follow the GP prior, we use the kernel derivative to obtain their cross covariance function (see \eqref{eq:cov-der-1}), with which to compute the GP conditional mean (conditioned on $\Ucal$) as the prediction. Take $\partial_{x_1} u$ and $\partial_{x_1x_2} u$ as examples. We have
\begin{align}
	\partial_{x_1} u (\x) = \partial_{x_1} \k(\x, \Gcal) \C^{-1} \vec(\Ucal), \;\;\; \partial_{x_1x_2} u (\x) = \partial_{x_1x_2} \k(\x, \Gcal) \C^{-1} \vec(\Ucal), \label{eq:der-example}
\end{align}
where $\k(\x, \Gcal) = [k(\x, \x'_1), \ldots, k(\x, \x'_M)]$ where $M = \prod_j M_j$ and all $\x'_j$ constitute $\Gcal$. We can accordingly predict the values of the all the relevant $u$ derivatives at $\Gcal$, and combine them to obtain the PDE (see \eqref{eq:pde}) evaluation at $\Zcal$, which we denote by $\Hcal$. To fit our GP model to the equation, we introduce another Gaussian likelihood,  
\begin{align}
	p(\0 | \Ucal) = \N(\0 | \vec(\Hcal), \tau_2^{-1}\I) \label{eq:eq-ll}
\end{align}
where $\0$ is an virtual observation, and $\tau_2>0$. Note that our modeling is similar to the recent GP solver~\citep{chen2021solving} and the GP framework that integrates differential equations~\citep{pmlr-v162-long22a}. However, there are two critical differences. First, rather than randomly sample the collocation points, we place all the collocation points on a grid. Second, rather than assign a multivariate Gaussian distribution jointly over the function values and all of its derivatives, we only model the distribution of the function values (at the grid). We then use the GP conditional mean to predict the derivative values. As we will discuss in Section \ref{sect:algo}, these modeling strategies, coupled with a product covariance function, can enable highly efficient and scalable computation, yet do not need any low rank approximation. 

\subsection{Product Covariance based on Spectral Mixture Kernel}
When the solution includes high frequencies or multi-scale information, \zhec{one naturally wants to estimate these target frequencies outright in the frequency domain. This is not straightforward for neural networks because we do not know its parametric form.}
 the commonly used kernels, such as the SE and Mat\'ern kernels, are incapable and ineffective, despite their popularity; see our experimental results at Section \ref{section:exp}. To address this problem, we consider the recent spectral mixture (SM) kernel~\citep{wilson2013gaussian}. Specifically, for any stationary kernel $k(\x, \x') = k(\x - \x')$, according to the Bochner’s theorem~\citep{bochner1959lectures}, the kernel can be represented by the inverse Fourier transform (IFT) of a positive, finite measure $S(\s)$, 
\begin{align}
	k(\x, \x')  = \int S(\s) \exp(i 2\pi \s^\top(\x - \x')) \d \s,  \label{eq:ift}
\end{align}
where $i$ indicates complex numbers.  The measure $S(\s)$ is called the spectral density or power spectrum of $k(\cdot)$. To boost expressivity, the SM kernel uses a Gaussian mixture to represent $S(\s)$,
\begin{align}
	S(\s) = \sum\nolimits_{q=1}^Q w_q \left(\N(\s | \bmu_q, \diag(\v_q)) + \N(\s | -\bmu_q, \diag(\v_q))\right). \label{eq:gmm}
\end{align} 
%For simplicity, we assume the covariance matrix of each Gaussian component is diagonal (but the result can be extended to non-diagonal cases). 
The two Gaussian components for each $q$ with the symmetric means $\bmu_q$ and $-\bmu_q$ are used to cancel out the imaginary part so as to obtain a real-valued kernel.  We can substitute \eqref{eq:gmm} into \eqref{eq:ift} and perform IFT. \cmt{The key intermediate result is that for each $q$, it can be derived that
\begin{align}
	\int \N(\s|\bmu_q, \diag(\v_q)) \exp\left(i 2\pi s^\top \boldeta\right) \d \s = \exp(i 2\pi \boldeta^\top \bmu_q)\cdot \exp\left(-2\pi^2 \boldeta^\top \diag(\v_q) \boldeta\right).
\end{align}
With this result, we can immediately obtain the SM kernel, }
Then we obtain the SM kernel
\begin{align}
	k_{\text{SM}}(\x, \x') = \sum\nolimits_{q=1}^Q w_q \exp\left(-2\pi^2 (\x- \x')^\top  \diag(\v_q) (\x - \x')\right)\cdot  \cos(2\pi (\x - \x')^\top \bmu_q).
\end{align}
We can see that the SM kernel includes a cosine function in each mixture component with frequency $\bmu_q$. The explicit injection of trigonometric kernels with different frequency parameters can effectively drive the learning of multiple or high frequencies within the target function.  The SM kernel has shown such success in standard GP training on time series data~\citep{wilson2013gaussian,chen2020incorporating,time-series-SM}. We therefore are enlightened to use the SM kernel in our GP-based PDE solver for solving high-frequency and multi-scale problems. 

Specifically, to enable low-cost, highly efficient computation, we introduce an SM kernel at each input dimension, and multiply them together to obtain our GP covariance function, 
\begin{align}
	\cov(f(\x), f(\x')) = k(\x, \x'|\Theta) = \prod\nolimits_{j=1}^d k_{\text{SM}}(x_j, x'_j|\btheta_q) \label{eq:cov-1}
\end{align}
where $\btheta_q = \{w_q, v_q, \mu_q\}$ and $\Theta = \{\btheta_q\}_{q=1}^Q$ are the kernel parameters. The product covariance here can lead to a Kronecker product structure in the covariance and cross-covariance matrices, which can greatly reduce the cost and accelerate the computation. We will discuss the details in Section \ref{sect:algo}. 

The standard SM kernel uses a Gaussian mixture to model the spectral intensity, which might not be robust enough~\citep{peel2000robust}. We therefore propose an extension by using the more robust student $t$ mixture. 
\begin{lem}
	With the following student $t$ mixture spectral density, 
\begin{align}
	S(s) = \sum_{q=1}^Q w_q \left(\text{St}(s; \mu_q, 4\pi^2\rho_q^2, 2\nu) +\text{St}(s; -\mu_q, 4\pi^2\rho_q^2, 2\nu) \right),
\end{align}
where $\text{St}(s;\mu, \lambda, \nu_0)$ is a student $t$ density with mean $\mu$, precision $\lambda$ and  the degree of freedom $\nu_0$. The corresponding stationary kernel is 
\begin{align}
	k_{\text{SMM}}(x, x') = \sum\nolimits_{q=1}^Q w_q \gamma_{\nu, \rho_q}(x, x') \cos(2\pi \mu_q (x - x'))
\end{align} 
where $\gamma_{\nu, \rho_q}(x, x') = \frac{2^{1-\nu}}{\Gamma(\nu)}\left(\sqrt{2\nu}\frac{|x - x'|}{\rho_q}\right)^{\nu} K_\nu(\sqrt{2\nu}\frac{|x - x'|}{\rho_q})$ is the Mat\'ern kernel with degree of freedom $\nu$ and length scale $\rho_q$, and $K_\nu$ is the modified Bessel function of the second kind.  
\end{lem}
We leave the proof in the Appendix. We name this kernel as a spectral Mat\'ern mixture (SMM) kernel. Hence, our second product covariance function is 
\begin{align}
		\cov(f(\x), f(\x')) = k(\x, \x'|\Theta) = \prod\nolimits_{j=1}^d k_{\text{SMM}}(x_j, x'_j|\btheta_q), \label{eq:cov-2}
\end{align}
where $\btheta_q = \{w_q, \mu_q, \rho_q\}$ and $\Theta = \{\btheta_q\}_{q=1}^Q$.

 
\section{Algorithm} \label{sect:algo}
According to \eqref{eq:prior-over-grid}, \eqref{eq:boundary-ll} and \eqref{eq:eq-ll}, 
the joint probability of our model is 
\begin{align}
	&p(\Ucal, \g, \0| \tau_1, \tau_2, \Theta) = p(\Ucal)p(\g | \u_b) p(\0 |\Ucal) = \N(\vec(\Ucal)|\0, \C) \N(\g | \u_b, \tau_1^{-1}\I)\N(\0|\vec(\Hcal), \tau_2^{-1}\I). \notag 
\end{align}
We maximize the log joint probability to estimate $\Ucal$, the kernel parameters $\Theta$, and the likelihood inverse variances $\tau_1$ and $\tau_2$. To allows us to flexibly adjust the influence of the boundary likelihood so as to reduce or balance the competition between the boundary and equation likelihoods~\citep{wang2020understanding,wang2020and}, we further introduce a free  hyper-parameter $\lambda_b>0$, and maximize the weighted log joint probability,  
\begin{align}
	\Lcal(\Ucal, \Theta, \tau_1, \tau_2) =& \log \N(\vec(\Ucal)|\0, \C) + \lambda_b \cdot \log \N(\g | \u_b, \tau_1^{-1}\I)  + \log \N(\0|\vec(\Hcal), \tau_2^{-1}\I) \notag \\
	=&-\frac{1}{2} \log|\C| - \frac{1}{2} \vec(\Ucal)^\top \C^{-1} \vec(\Ucal) + \lambda_b\left[\frac{N_b}{2} \log \tau_1 - \frac{\tau_1}{2} \|\u_b - \g\|^2\right] \notag \\
	& +\frac{M}{2} \log \tau_2 - \frac{\tau_2}{2} \|\vec(\Hcal)\|^2 + \text{const}. \label{eq:obj}
\end{align}
Naive computation of $\Lcal$, however, is extremely expensive when the grid is dense, namely, $M$ is large. That is because the covariance matrix $\C$ is between all the grid points, of size $M \times M$ ($M = \prod_j M_j$). Also, to obtain $\Hcal$, we  need to compute the cross-covariance between every needed derivative in the PDE operator and $u$ across all the $M$ grid points. Consequently, the naive computation of the log determinate and inverse of $\C$ (see \eqref{eq:obj} ) and the required cross-covariance take the time and space complexity $\Ocal(M^3)$ and $\Ocal(M^2)$, respectively, which can be infeasible even when each $M_j$ is relatively small. For example, when $d=3$, and $M_1 = M_2  = M_3 = 100$, we have $M=10^6$ and the computation of $\C$ will be too costly to be practical (on most computing platforms). 

Thanks to that (1) our prior distribution \eqref{eq:prior-over-grid} is only on all the function values at the grid, and (2) our covariance function is a product over each input dimension (see \eqref{eq:cov-1} and \eqref{eq:cov-2}). We can obtain a Kronecker product structure in $\C$,  namely, $\C =  \C_1 \kron \ldots \kron \C_d$, 
%However, since our prior distribution \eqref{eq:prior-over-grid} is only on all the function values at the grid, and our covariance function is a product over each input dimension (see \eqref{eq:cov-1} and \eqref{eq:cov-2}), we can derive a Kronecker product structure in $\C$,  %and in the cross covariance matrix between the values of any $u$ derivative at the grid and $\Ucal$.  
%\begin{align}
%	\C =  \C_1 \kron \ldots \kron \C_d
%\end{align}
where $C_j = \kappa(\h_j, \h_j)$ is the kernel matrix on $\h_j$ --- the locations at input dimension $j$, of size $M_j \times M_j$, and $\kappa$ is either $k_{\text{SM}}$ or $k_{\text{SMM}}$.  Using the Kronecker product properties~\citep{minka2000old}, we obtain
\begin{align}
	\log |\C| &= \sum\nolimits_{j=1}^d \frac{M}{M_j} \log | \C_j|, \notag \\
	 \C^{-1} \vec(\Ucal) &= \left(\C_1^{-1} \kron \ldots \kron \C_d^{-1}\right) \vec(\Ucal) = \vec\left(\Ucal \times_1 \C_1^{-1} \times_2 \ldots \times_d \C_d^{-1} \right), \label{eq:comp-c}
\end{align}
where $\times_j$ is the tensor-matrix product at mode $j$. Accordingly, we can first compute the local log determinant and inverse at each input dimension (\ie for each $\C_j$), which reduces the time and space complexity to $\Ocal(\sum_{j=1}^d M_j^3)$ and $\Ocal(\sum_{j=1}^d M_j^2)$, respectively. Then we perform the multilinear operation in the last line of \eqref{eq:comp-c}, \ie sequentially multiplying the array $\Ucal$ with each $C_j^{-1}$, which takes the time complexity $\Ocal\left((\sum_{j=1}^d M_j) M\right)$. The computational cost is  dramatically reduced. %\zhec{add an example?}

Furthermore, since our product covariance function is factorized over each input dimension, the cross covariance between any derivative of $u$ and $u$ itself still maintains a product form --- because only the kernel(s) at the corresponding input dimension(s) need to be differentiated. For example, 
\begin{align}
		&\cov(\partial_{x_1x_2} u(\x), u(\x')) = \partial_{x_1x_2} \kappa(\x, \x') = \partial_{x_1x_2}\prod\nolimits_{j} \kappa(x_j, x_j')\notag \\
		&= \partial_{x_1} \kappa(x_1, x_1') \cdot \partial_{x_2}\kappa(x_2, x_2') \cdot \prod\nolimits_{j>2} \kappa(x_j, x_j'). 
\end{align}
Accordingly, we can also obtain Kronecker product structures in predicting each derivative of $u$.  Take $\partial_{x_1x_2} u$ as an example. According to \eqref{eq:der-example}, we can derive that 
\begin{align}
	&\partial_{x_1x_2} u (\x) = \left(\partial_{x_1} \k(x_1, \h_1)  \kron  \partial_{x_2} \k(x_2, \h_2) \kron \ldots \kron  \k(x_d, \h_d)\right)\left(\C_1^{-1} \kron \ldots \kron \C_d^{-1}\right)\vec(\Ucal) \notag \\
	&=\left(\partial_{x_1} \k(x_1, \h_1) \C_1^{-1}  \kron \partial_{x_2} \k(x_2, \h_2) \C_2^{-1} \kron  \ldots \kron  \k(x_d, \h_d)\C_d^{-1}\right) \vec(\Ucal)  \notag \\
	&=\vec\left(\Ucal \times_1 \partial_{x_1} \k(x_1, \h_1) \C_1^{-1}   \times_2 \partial_{x_2} \k(x_2, \h_2) \C_2^{-1}  \times_3 \k(x_3, \h_3) \C_3^{-1} \times_4 \ldots \times_d \k(x_d, \h_d)\C_d^{-1}\right). \notag 
\end{align}
Denote the values of $\partial_{x_1x_2} u $ at the grid $\Mcal$ by $\partial_{x_1x_2} \Ucal \overset{\Delta}{=} \{\partial_{x_1x_2} u (\x) | \x \in \Mcal\}$. Then it is straightforward to obtain
\begin{align}
	\partial_{x_1x_2} \Ucal = \Ucal \times_1 \nabla_1\C_1 \times_2  \nabla_1\C_2
\end{align}
where $\nabla_1$ means taking the derivative w.r.t the first input variable, and we have 
$\nabla_1\C_1 = [\partial_{h_{11}} \k(h_{11}, \h_1); \ldots; \partial_{h_{1M_1}} \k(h_{1M_1}, \h_1)]$ and $\nabla_1\C_2 = [\partial_{h_{21}} \k(h_{21}, \h_2); \ldots; \partial_{h_{2M_2}} \k(h_{2M_2}, \h_2)]$. Hence, we just need to perform two tensor-matrix products, which takes $\Ocal((M_1 + M_2)M)$ operations, and is efficient and convenient. Similarly, we can  compute the prediction of all the associated $u$ derivatives in the PDE operator, with which we can obtain $\Hcal$ --- the PDE evaluation at the grid in \eqref{eq:obj}. Once we can efficiently compute \eqref{eq:obj}, we can use automatic differentiation libraries to calculate the gradient, and apply any gradient-based optimization to maximize \eqref{eq:obj}. 

\noindent\textbf{Algorithm Complexity.} The time complexity of our algorithm is $\Ocal(\sum_{j}M_j^3 + (\sum_{j}M_j)M)$. The space complexity is $\Ocal(\sum_{j}M_j^2 + M)$, including the storage of the covariance matrix at each input dimension, and the solution estimate at the grid $\Gcal$, namely $\Ucal$. 

%\partial_{x_1} u (\x) = \partial_{x_1} \k(\x, \Gcal) \C^{-1} \vec(\Ucal), \;\;\; \partial_{x_1x_2x_2} u (\x) = \partial_{x_1x_2x_2} \k(\x, \Gcal) \C^{-1} \vec(\Ucal) \label{eq:der-example}

%we can derive a Kronecker product structure in $\C$,  %and in the cross covariance matrix between the values of any $u$ derivative at the grid and $\Ucal$.  
%Thanks to our prior distribution over the function values (only) on the grid, and thanks to our product covariance design (see \eqref{eq:cov-1} and \eqref{eq:cov-2}), 

 

==> model.tex <==
%background --> Model --> Algorithm --> Related Work 
%model --> start setting, and talk about a grid --> mention this is useful and will discuss about it later --> and then go to the next 
%GP prior 
%\vspace{-0.13in}
%1. Gaussian process 2. horseshoe
\section{Background}\label{sect:bk}
%Gp part can still be tuncated, maybe rmeoving the noisy likelihood, just mention the kernel interpolation 
\noindent \textbf{Kernel Regression and Gaussian processes} \zhec{freq view, interpolation, connection to GP} are powerful nonparametric function estimators in that they do not assume any parametric form of the target function, and can flexibly  capture the complexity of the function according to the data, \eg from simple linear, to quadratic, and to highly nonlinear, and hence can prevent both underfitting and overfitting. Specifically, GP models assume the target function $f: \mathbb{R}^d \rightarrow \mathbb{R}$ is sampled from a  Gaussian process, $f \sim \gp(m(\cdot), \kappa(\x, \x'))$, where $m(\cdot)$ is the mean function,  and $\kappa(\cdot, \cdot)$ is the covariance function,  \ie $\cov(f(\x), f(\x')) = \kappa(\x, \x')$, which characterizes how the function values are correlated according to their inputs.  In practice, one often sets $m(\cdot)$ to the constant zero and chooses a kernel function as the covariance function. For example, a popular choice is the Square Exponential (SE) kernel, $\kappa(\x, \x') = \exp\left(-\frac{1}{\eta}\|\x - \x'\|^2\right)$ where $\eta$ is the length-scale parameter. Under the GP prior, the values of the sampled function at an arbitrary finite set of inputs, $\f = [f(\x_1), \ldots, f(\x_N)]$, follow a multi-variate Gaussian distribution, $p(\f) = \N(\f|\0, \K)$ where $[\K]_{ij} = \kappa(\x_i, \x_j)$. Suppose we have collected the training dataset $\Dcal = \{(\x_1, y_1), \ldots, (\x_N, y_N)\}$. Given $\f$, we use a noise model to fit the data while capturing the possible noises in the data. For continuous observations,  a commonly used model is the Gaussian noise model, $p(\y|\f) = \N(\y | \f, \sigma^2\I)$ where $\sigma^2$ is the noise variance and $\y = [y_1; \ldots ; y_N]$. \cmt{The marginal likelihood of data (model evidence) is therefore 
\begin{align}
p(\y|\X) = \N(\y|\0, \K + \sigma^2\I).
\end{align}
One can maximize the marginal likelihood to estimate the kernel parameters and noise variance.}  Given a test input $\x^*$, since $[\y; f(\x^*)]$ jointly follow a multi-variate Gaussian distribution, we can immediately obtain the predictive distribution as a conditional Gaussian, 	$p\big(f(\x^*)|\X, \y\big) = \N\big(f(\x^*)|\mu(\x^*), v(\x^*)\big)$,
%\begin{align}
%	p\big(f(\x^*)|\X, \y\big) = \N\big(f(\x^*)|\mu^*, v^*\big),
%	\label{eq:predictive}
%\end{align}
where $\mu(\x^*) = \k_*^\top(\K + \sigma^2\I)^{-1}\y$, $v(\x^*)=\kappa(\x^*, \x^*) - \k_*^\top(\K + \sigma^2\I)^{-1}\k_*$ and  $\k_* = [\kappa(\x^*, \x_1), \cdots,\kappa(\x^*, \x_N)]^\top$. Note that the conditional mean $\mu(\x^*)$ is also known as the kernel interpolation from the data points $\y$.
 %We can see that due to the closed-form posterior, GP models are easy and convenient to quantify and reason under uncertainty. 

%put HS here --- then talk about the regularized horseshoe prior in the paper 
\noindent \textbf{Horseshoe prior (HS)}~\citep{carvalho2009handling} is a Bayesian sparse prior distribution that can be used to identify dominant patterns/signals from data. Take basis selection as an example. Suppose we have $M$ bases, $\{\phi_j(\x)\}_{j=1}^M$, with which we want to represent the target function as $f(\x) = \sum_{j=1}^M w_j \phi_j(\x)$. We can assign a HS prior over each weight $w_j$ to select the dominant/relevant bases and prune the irrelevant ones. The HS prior is a scaled mixture of Gaussian, 
\begin{align}
	p_\text{HS}(w_j) = \int  \N(w_j|0, \lambda_j^2 s^2) C^+(\lambda_j|0, a_0) C^+(s|0, a_1) \d \lambda_j \d s, \label{eq:hs}
\end{align}
where $C^+$ is the Half-Cauchy density with a flat tail, $C^+(x | 0,a) = \frac{2}{\pi a (1 + x^2/a^2)} \cdot \mathds{I}(x> 0)$ where $\mathds{1}(\cdot)$ is the indicator function, $\lambda_j$ is a local scale specific for basis $j$ and $s$ the global scale shared by all the bases. HS density has an infinitely tall spike at zero, which means it can provide a strong shrinkage effect over the weight in the posterior if the basis is irrelevant. On the other hand, by mixing with Half-Cauchy, the HS prior has flat, Cauchy-like tails. The flat tails imply a mild regularization.  Hence, if the basis is relevant, the weight $w_j$ can escape from being shrunk  and be freely learned from data. This selective shrinkage effect is more favorable than $L_1$ regularization (or Laplace prior), which  uniformly shrinks all the weights, no matter if the corresponding bases are relevant or not. 

%problem def, a spatial-temporal system, u(t,x_1, x_2, ... x_m), when m= 0, it reduces to ODE  --> candidate operators --> derivaties p(u_Zcal) --> derviatves D_1, .. D_a--> kernel interpolation --> kernel differentiation & interpolation --> s&s --> joint distribution 

%algorithm: we propose EM algorihtm. First, if we use a product kernel, like SE kernel, the covariance can be represtned by a Kronecerk product ....---> convenince in computing deriative covariance  Second, we use the EP framework. basic description, link to appendix. introduce the approximation, and then udpate, algorithm table 
\section{Model}
To discover the underlying governing equation from scarce, noisy data, we propose a Bayesian equation discovery model based Gaussian processes.  Without loss of generality, we consider a spatial-temporal system. We denote  the response (or solution) function by $u(t,x_1, \ldots, x_m)$. Note that when $m=0$, it reduces to an ODE system. Given a small collection of measurement data, $\Dcal = \{(\x_1, y_1), \ldots, (\x_P, y_P)\} $, we aim to learn $u$ and the governing equation about $u$. To this end, we first prepare a dictionary of candidate operators $\Fcal = \{\psi_1, \ldots, \psi_M\}$, which consists of basic differentiation operators, such as $D_0 [u]$, $D_{1} [u]$, and $D_{22} [u]$, their linear/nonlinear combinations, and composition with other functions: $u D_0 [u]$, $u D_1 [u]$,  $u$, $u^2$, $u^3$, $\cos(u)$, $\sin(u)$, \etc Here $D_\a [u]$ means the partial derivatives of $u$ w.r.t the input variable(s) indexed by $\a$, \eg  $D_0[u]  = \frac{\partial u}{\partial t}$, $D_{1}[u]  = \frac{\partial u}{\partial x_1}$, and $D_{122}[u] =\frac{\partial^3 u}{\partial x_1 \partial x_2^2}$. 
We assume the governing equation can be expressed as a linear combination of  a small set of operators from $\Fcal$,
%To discover the underlying governing equation from scarce, noisy data, we propose a Gaussian process (GP) based model. Without loss of generality, we consider a 1d spatial-temporal system to explain the idea.  We denote  the response (or solution) function by $u(t,x)$. Given a small collection of measurement data, $\Dcal = \{((t_1, x_1), y_1), \ldots, ((t_N, x_N), y_N)\} $, we aim to learn $u$ and the governing equation about $u$. To this end, similar to~\citep{brunton2016discovering,chen2021physics}, we first prepare a dictionary of candidate operators $\Fcal = \{\psi_1, \ldots, \psi_M\}$, which consists of basic differentiation operators, such as $u_x$, $u_t$, and $u_{xx}$, their linear/nonlinear combinations, and composition with other functions: $u u_t$, $u u_x$,  $u$, $u^2$, $u^3$, $\cos(u)$, $\sin(u)$, \etc We assume the governing equation can be represented by a linear combination of  a small set of operators from the dictionary,
\begin{align}
	\frac{\partial u}{\partial t} - \sum\nolimits_{j=1}^M w_j \psi_j[u] = 0 \label{eq: form}
\end{align}
where most of the coefficients $\{w_j\}$ are zero. 
%this sentence can be removed
 Note that the linear structure does not restrict our flexibility of finding nonlinear equations, because the dictionary can include nonlinear operators. The framework can account for unknown source terms by adding the corresponding candidate functions into $\Fcal$ to explain the source.

To estimate the target function $u$ and perform operator selection in \eqref{eq: form}, we create a dense grid in the domain of interest, and consider estimating the function values at the grid. Denote the inputs  at each dimension by $\z_1, \ldots, \z_{m+1}$, where each $\z_j$ includes $N_j$ inputs. The grid points are 
\begin{align}
	\Zcal = \z_1 \times \cdots \times \z_{m+1} = \{(z_1, \ldots, z_{m+1}) | z_j \in \z_j, 1 \le j \le m+1\}.
\end{align}
Denote by $\Ucal$ the values of $u(\cdot)$ at the grid points $\Zcal$. Hence $\Ucal$ is a $m+1$ dimensional tensor, of size $N_1 \times \ldots \times N_{m+1}$.  We place a GP prior over $u$, and $\Ucal$ therefore follows a multi-variate Gaussian prior distribution, 
\begin{align}
	p(\Ucal) = \N(\vec(\Ucal)| \0, \K_{\Zcal\Zcal}) \label{eq:prior-u}
\end{align}
where $\K_{\Zcal\Zcal}$ is the kernel matrix computed from $\Zcal$.

Given $\Ucal$, we first obtain the function values at the training inputs $\Xcal = \{\x_1, \ldots \x_P\}$ via kernel interpolation, 
\begin{align}
	f_n \overset{\Delta}{=} u(\x_n) = \kappa(\x_n, \Zcal) \K_{\Zcal\Zcal}^{-1} \vec(\Ucal), \;\;\; 1 \le n \le P  \label{eq:kint-1}
\end{align}
with which we sample the observed outputs from a Gaussian noise model, %$p(\y|\u) = \N(\y|\u, \sigma_0^2I)$
\begin{align}
	p(\y|\f) = \N(\y|\f, \tau_1^{-1}\I ) \label{eq:gp-ll}
\end{align}
where $\f = [f_1, \ldots f_P]^\top$, and $\tau_1$ is the noise inverse variance. 

Next, to select the operators from $\Fcal$ and to identify the equation, we obtain all the needed derivatives values of $u$ on $\Zcal$, so as to obtain the evaluation of every candidate operator on $\Zcal$. For example, suppose one operator is $\psi [u] =  D_{jk}[u] u$. We need to obtain the values of $D_{jk}[u]$ on $\Zcal$ and then obtain the values of  $\psi[u]$ on $\Zcal$. 
This is can be done via kernel differentiation and interpolation. Specifically, consider arbitrary inputs $\balpha$ and $\balpha'$ in the domain. Suppose we want to obtain $D_{jk} [u(\balpha)]$ given $\Ucal$. Since $u(\cdot)$ is a GP, its derivative $D_{jk}[u]$ is a also a GP, and the covariance/kernel between $D_{jk} u(\balpha)$ and $u(\balpha')$ is derived from the kernel differentiation at the same input variables with respect to which we take the derivative, 
\begin{align}
	\cov(D_{jk} [u(\balpha)], u(\balpha')) = D_{jk} [\kappa(\balpha, \balpha')]  = D_{jk} [ \kappa(\alpha_1, \ldots \alpha_{m+1}, \alpha'_1, \ldots, \alpha'_{m+1})]. \label{eq:ker-diff}
\end{align}
\cmt{Note that we expand the input vectors to the kernel function $\kappa$ to be more clear.} Therefore, we can use the new kernel to obtain the interpolation for $D_{jk}[u(\balpha)]$ from $\Ucal$, 
\begin{align}
	D_{jk}[u(\balpha)] = D_{jk} [\kappa(\balpha, \Zcal)] \K_{\Zcal\Zcal}^{-1} \vec(\Ucal) \label{eq:kint-2}
\end{align}
where $D_{jk}[\kappa(\balpha, \Zcal)]  = \left[D_{jk}[\kappa(\balpha, \balpha_1')], \ldots, D_{jk}[\kappa(\balpha, \balpha_N')]\right]$, all $\balpha'_n \in \Zcal$ and  $N = \prod_{j=1}^{m+1} N_j$. 
%$D_{jk}[\kappa(\z, \Zcal)] = \{D_{jk}[\kappa(\z, \z')]|\z' \in \Zcal\}$.

 Let us denote the evaluated values of each candidate operator on $\Zcal$  by $\bphi_1, \ldots, \bphi_M$. To identify the operators in the governing equation, for each $\bphi_j$, we use a spike-and-slab prior to sample a selection indicator $s_j$ and the operator coefficient $w_j$, 
 \begin{align}
 	p(s_j) = \text{Bern}(s_j|\rho_0) = \rho_0^{s_j}(1 - \rho_0)^{1 - s_j}, \;\;p(w_j | s_j) = s_j\N(w_j|0, \sigma_0^2) + (1 - s_j)\delta(w_j), \label{eq:ss-2}
 \end{align}
 We then sample a virtual dataset $\wy = \0$, given the candidate operators' evaluation results  on $\Zcal$, 
\begin{align}
	p(\wy|\bPhi, \w) = \N\left(\wy|\h - \bPhi \w, \tau_2^{-1} \I\right) \label{eq:vll}
\end{align}
where $\bPhi = [\bphi_1, \ldots, \bphi_M]$, $\w = [w_1, \ldots, w_M]^\top$, and $\h$ is $\frac{\partial u}{\partial t}$ evaluated at $\Zcal$. Note that each $\bphi_j$ ($1\le j \le M$) and $\h$ have been flattened into a vector. The equation likelihood \eqref{eq:vll} measures how consistent the selected equation is with the estimate of $\Ucal$ and the operators. During the learning,  the data likelihood~\eqref{eq:gp-ll} and equation likelihood~\eqref{eq:vll} will synergize to learn $\Ucal$ and the underlying equation.    

%The supervised signal comes from the data likelihood  \eqref{eq:gp-ll}, and propagate through the kernel interpolation \eqref{eq:kint-1} and \eqref{eq:kint-2}. The equation likelihood \eqref{eq:vll} combined with the spike-and-slab prior \eqref{eq:ss-2} then identify the operators and their coefficients. During the learning, the data likelihood and equation likelihood will synergize for the estimation of $\Ucal$ and the equation identification.  
%evaluations $\{\bphi_j\}$, computed based on $\g$, and $\g$ are coupled with $\u$ in the GP prior \eqref{eq:gp-joint}. Via fitting the data by \eqref{eq:gp-ll}, the supervised information is propagated to $\g$ and then each $\bphi_j$. 
The joint distribution of our model is given by
\begin{align}
	%p(\u, \g, \y, \wy, \w) =  \N\left([\u; \g]|\0, \bSigma\right) \prod\nolimits_{j} p_{\text{HS}}(w_j)  \N(\y|\f, \sigma_0^2\I) \N\left(\wy|\brho - \sum\nolimits_{j} w_j  \bphi_j, \sigma_1^2\I\right).
	p(\Ucal, \f, \y, \w, \s, \wy) &= \N(\vec(\Ucal)| \0, \K_{\Zcal\Zcal})\cdot \prod\nolimits_{j=1}^M  \text{Bern}(s_j|\rho_0) \left( s_j\N(w_j|0, \sigma_0^2) + (1 - s_j)\delta(w_j)\right) \notag \\
	&\cdot \N(\y|\f, \tau_1^{-1}\I) \N\left(\wy|\h - \bPhi \w, \tau_2^{-1} \I\right). \label{eq:joint-2}
\end{align} 
 where $\s = [s_1, \ldots, s_M]^\top$. 

\cmt{
Denote by $\u$ the target function values at the training inputs, and by $\g$ the required derivatives evaluated on the collocation points $\Zcal$. Using the covariance function derived by kernel operation (see \eqref{eq:kernel-diff-int}), we  can construct a multivariate Gaussian prior distribution for $\u$ and $\g$, 
\begin{align}
	p(\u, \g) = \N([\u;\g]| 0, \bSigma), \label{eq:gp-joint}
\end{align}
where $\bSigma$ is the covariance matrix computed via \eqref{eq:kernel-diff-int}.  Given $\u$, we then sample the observed training outputs from a Gaussian noise model, %$p(\y|\u) = \N(\y|\u, \sigma_0^2I)$
\begin{align}
	p(\y|\u) = \N(\y|\u, \sigma_0^2\I) \label{eq:gp-ll}
\end{align}
where $\sigma_0^2$ is the noise variance. Accordingly, via posterior inference,  we can fit the data while accounting for the noise level. Given $\g$, we can obtain the evaluation of every operator $\psi_j[u] \in \Fcal$  on $\Zcal$. Let us denote the evaluated values with each operator  by $\bphi_1, \ldots, \bphi_M$. To identify the operators in the governing equation, we sample a coefficient $w_j$ for each operator $\psi_j$, from a horse-shoe prior (see \eqref{eq:hs}), which strongly encourages sparsity, 
\begin{align}
	p(\w) = \prod\nolimits_j p_{\text{HS}}(w_j),
\end{align}
where $\w = [w_1, \ldots, w_M]$. We then sample a virtual dataset $\wy = \0$, given the candidate operators' evaluation results  on $\Zcal$, 
\begin{align}
	p(\wy|\bPhi, \w) = \N\left(\wy|\brho - \sum\nolimits_{j} w_j\bphi_j, \sigma^2_1 \I\right) \label{eq:vll}
\end{align}
where $\bPhi$ denote all the evaluation results, $\brho$ is $u_t$ evaluated at $\Zcal$. Note that $\brho$ is a part of $\g$ and sampled from \eqref{eq:gp-joint}. 
The supervised signal comes from the operator evaluations $\{\bphi_j\}$, computed based on $\g$, and $\g$ are coupled with $\u$ in the GP prior \eqref{eq:gp-joint}. Via fitting the data by \eqref{eq:gp-ll}, the supervised information is propagated to $\g$ and then each $\bphi_j$. The horse-shoe prior density has an infinitely tall spike at the zero and heavy, Cauchy-like tails (see Sec. \ref{sect:bk}). Therefore, if an operator $j$ is irrelevant, the data will guide the coefficient $w_j$ to move toward zero,  $w_j$ will bear a severe shrinkage from the HS prior, making its posterior concentrate around zero. Otherwise, if the operator is dominant,  the data will guide $w_j$ move away from zero, where the HS prior only puts a tiny  regularization (flat tails).  Hence, $w_j$ will be fully estimated from data. In this way, our model enables data-driven operator selection and equation identification. The joint distribution of our model is given by
\begin{align}
	p(\u, \g, \y, \wy, \w) =  \N\left([\u; \g]|\0, \bSigma\right) \prod\nolimits_{j} p_{\text{HS}}(w_j)  \N(\y|\f, \sigma_0^2\I) \N\left(\wy|\brho - \sum\nolimits_{j} w_j  \bphi_j, \sigma_1^2\I\right).
\end{align}
%where $\wy = \0$ is the virutal data. 
}
%the goal, posterior dist. of the selection indicators and operator coefficients, ; next to decouple the strong relationshp, we use the whitening trick  
\section{Algorithm}
We now present the model estimation algorithm. Given the training data $\Dcal$, we aim to estimate the function values at the grid $\Zcal$, \ie $\Ucal$, the kernel parameters $\btheta$, and the posterior distribution of the selection indicators $\s$ and the operator coefficients $\w$. This is challenging, because the spike-and-slab prior in \eqref{eq:ss-2} mixes binary and continuous random variables, making the posterior distribution analytically intractable. In addition, when the grid is dense, \ie the number of grid points  is large, computing the covariance matrix $\K_{\Zcal\Zcal}$ in the prior (see \eqref{eq:prior-u}) and kernel interpolation (see \eqref{eq:kint-1} and \eqref{eq:kint-2}) is prohibitively expensive. To address these issues, we introduce a factorized approximation to the spike-and-slab prior for efficient posterior estimation. We  leverage the grid structure in $\Ucal$, and use a product kernel to evade computing the full covariance matrix. Bases on these methods, we develop an efficient expectation-propagation expectation-maximization (EP-EM) algorithm. In each iteration, our algorithm performs two steps. In the E step, we fix $\Ucal$ and $\btheta$, and use the expectation propagation (EP) framework~\citep{minka2001expectation} to estimate the posterior of $\s$ and $\w$. In the M step, we maximize the expected log joint probability to update $\Ucal$ and $\btheta$. The alternating of the E and M steps keeps mutually improving the function estimate and equation discovery until convergence. 

Specifically, in the E step,  we use the expectation propagation (EP) framework to estimate $p(\s, \w|\Dcal, \wy)$. EP approximates each non-exponential-family factor in the joint probability with an exponential-family term. Then in the approximate joint probability, every factor is in the exponential family and we can obtain a closed-form posterior approximation, because the exponential family is closed under multiplication. EP iteratively updates each factor approximation until convergence. A more detailed introduction to  EP is given in the appendix. To conduct EP for our model,  we introduce a factorized approximation to the mixture term in the spike-and-slab prior \eqref{eq:ss-2}, 
\begin{align}
	s_j\N(w_j|0, \sigma_0^2) + (1 - s_j)\delta(w_j) \approx c_j \text{Bern}(s_j|\sigma({\rho_j}))\N(w_j|\mu_j, v_j), \;\; 1 \le j \le M \label{eq:ss-approx}
\end{align}
where $\sigma(\cdot)$ is the sigmoid function, and $c_j>0$ is a constant scale. Note that all the other terms in the joint probability \eqref{eq:joint-2} are within the exponential family. Substituting \eqref{eq:ss-approx} into \eqref{eq:joint-2}, we can obtain the approximated posterior, 
\begin{align}
	p(\s, \w|\Dcal, \wy) \approx q(\s, \w) = \prod\nolimits_{j=1}^M \text{Bern}(s_j|\sigma(\widehat{\rho}_j)) \cdot \N(\w|\bbeta, \bSigma) \label{eq:qws}
\end{align}
where $\widehat{\rho}_j = \sigma^{-1}(\rho_0) + \rho_j$, $\bSigma = \left(\text{diag}^{-1}(\v) + \tau_2\bPhi^\top \bPhi\right)^{-1}$, and $\bbeta = \bSigma\left(\frac{\bmu}{\v} + \tau_2 \bPhi^\top \h\right)$.
%\begin{align}
%	\widehat{\rho}_j = \sigma^{-1}(\rho_0) + \rho_j, \;\; \bSigma = \left(\text{diag}^{-1}(\v) + \tau_2\bPhi^\top \bPhi\right)^{-1}, \;\; \bbeta = \bSigma\left(\frac{\bmu}{\v} + \tau_2 \bPhi^\top \h\right)
%\end{align}
Here $\bmu = [\mu_1, \ldots, \mu_M]^\top$ and $\v = [v_1, \ldots, v_M]^\top$.  The update of each approximation factor \eqref{eq:ss-approx} is performed by three steps: message deletion, projection via moment matching and message update. In each iteration, we update each  factor in parallel. We provide the details in Appendix (see XX).  


In the M step, we maximize the expected log joint probability under the current posterior estimate $q(\s, \w)$ to update $\Ucal$ and the kernel parameters $\btheta$, 
\begin{align}
	\Lcal = \log|\K_{\Zcal\Zcal}| - \frac{1}{2}\vec(\Ucal)^\top \K_{\Zcal\Zcal}^{-1} \vec(\Ucal) - \frac{1}{2}\tau_1 \| \y - \f\|^2   - \frac{1}{2}\tau_2\EE_q\left[ \|\h - \bPhi \w\right\|^2] + \text{const} \label{eq:log-ll}
\end{align}
  One major bottleneck is the computation regarding the huge covariance matrix $\K_{\Zcal\Zcal}$, especially in the kernel interpolation \eqref{eq:kint-1} and \eqref{eq:kint-2}. To address this issue, we observe that the function values $\Ucal$ are on the grid $\Zcal$.  If we use a product kernel
\begin{align}
	\kappa(\balpha, \balpha') = \prod\nolimits_{j=1}^{m+1} \kappa(\alpha_j, \alpha_j'),
\end{align}
the prior covariance matrix in \eqref{eq:prior-u} will become a Kronecker product of the kernel matrices in each input dimension, 
\begin{align}
	\K_{\Zcal\Zcal} = \K_1 \kron \ldots \kron \K_{m+1}
\end{align}
where $\K_j = \kappa(\z_j, \z_j)$ is the $N_j \times N_j$ kernel matrix at input dimension $j$ ($1 \le j \le m+1$). Accordingly, we can utilize the Kronecker product properties and tensor algebra to  compute the related terms highly efficiently, without the need for computing the full matrix $\K_{\Zcal\Zcal}$.  Note that the popular SE kernel, which was mainly used in our experiments, is a product kernel. We can also construct a product kernel based on other kernels, such as the Matern kernel.  
To obtain the values of a required derivative on $\Zcal$, we first observe that the corresponding kernel differentiation still gives rise to a product kernel. That is because each differentiation is only taken in one term of the product. Take $D_{jk}[u]$ ($j < k$) in \eqref{eq:ker-diff} as an example. We can derive that
\begin{align}
	&\cov(D_{jk} [u(\balpha)], u(\balpha')) = D_{jk} [\kappa(\balpha, \balpha')]  = D_{jk} [ \prod\nolimits_t k(\alpha_t, \alpha_t')] \notag \\
	&= D_1[\kappa(\alpha_j, \alpha_j')] \cdot D_1[\kappa(\alpha_k, \alpha_k')]\cdot \prod\nolimits_{t\neq j, k} \kappa(\alpha_t, \alpha_t').
\end{align}
To compute $D_{jk}[u(\Zcal)]$, namely, the values of $D_{jk}[u]$ on all the grid points $\Zcal$, we therefore have
\begin{align}
\vec\left(D_{jk}[u(\Zcal)]\right) = \left(\H_{<j} \kron D_1 [\kappa(\z_j, \z_j)] \kron \H_{>j,<k}  \kron D_1 [\kappa(\z_k, \z_k)] \kron \H_{>k} \right) \K_{\Zcal\Zcal}^{-1}  \vec(\Ucal) \label{eq:der-grid}
\end{align}
where $\H_{<j} = \K_1 \kron \ldots \kron \K_{j-1}$, $\H_{>j, <k} = \K_{j+1} \kron \ldots \kron \K_{k-1}$, $\H_{>k} = \K_{k+1} \kron \ldots \kron \K_{m+1}$,  $D_1 \kappa(\z_j, \z_j)$ is an $N_j \times N_j$ matrix where each row is $D_1 [\kappa(z_{jn}, \z_j)]$ ($1 \le n \le N_j$), and $D_1 \kappa(\z_k, \z_k)$ is an $N_k \times N_k$ matrix where each row is $D_1[\kappa(z_{kn}, \z_k)]$. 

 According to the Kronecker product property, we have $\K_{\Zcal\Zcal}^{-1} = \K_1^{-1} \kron \ldots \kron \K_{m+1}^{-1}$. Substituting this into  \eqref{eq:der-grid}, we obtain
\begin{align}
\vec\left(D_{jk}[u(\Zcal)]\right) &= \left(\I \kron \ldots \kron \I  \kron D_1 \kappa(\z_j, \z_j)  \kron \I \kron \ldots \kron \I \kron  D_1 \kappa(\z_k, \z_k) \kron \I \kron  \ldots \kron \I  \right)\vec(\Ucal) \notag \\
&=\vec\left( \Ucal \times_j D_1 [\kappa(\z_j, \z_j)  \K_j^{-1}]  \times_k  [D_1 \kappa(\z_k, \z_k) \K_k^{-1}] \right), \label{eq:tucker}
\end{align}
\cmt{
\begin{align}
	&\vec\left(D_{jk}[u(\Zcal)]\right) = \left(\H_{<j} \kron D_1 \kappa(\z_j, \z_j) \kron \H_{(j+1, k-1)}  \kron D_1 \kappa(\z_k \z_k) \kron \H_{>k} \right) \K_{\Zcal\Zcal}^{-1}  \vec(\Ucal) \notag \\
	&= \left(\H_{<j}\H_{<j}^{-1} \kron D_1 \kappa(\z_j, \z_j)  \K_j^{-1} \kron \H_{(j+1, k-1)} \H_{(j+1, k-1)}^{-1}  \kron D_1 \kappa(\z_k \z_k) \K_k^{-1} \kron \H_{k+1} \H_{>k}^{-1}\right) \vec(\Ucal) \notag \\
	&= \vec\left( \Ucal \times_j D_1 \kappa(\z_j, \z_j)  \K_j^{-1}  \times_k  D_1 \kappa(\z_k \z_k) \K_k^{-1} \right)
\end{align}
}
where $\times_j$ is the tensor-matrix product at mode $j$.  The second line of \eqref{eq:tucker} is from the definition of Tucker operator in the tensor algebra~\citep{kolda2006multilinear}. We can see that, the computation only performs kernel differentiation and matrix inverse at each individual input dimension involved in the derivative operator, and we never need to compute and invert the full matrix $\K_{\Zcal\Zcal}$. In this way, we can dramatically promote the efficiency and scale to  a large number of grid points.  We can follow a similar approach to obtain the values of all the required derivatives on $\Zcal$, each $f_n$ in \eqref{eq:kint-1}, and $\vec(\Ucal)^\top \K_{\Zcal\Zcal}^{-1} \vec(\Ucal)$ in the log prior of $\Ucal$ (see \eqref{eq:log-ll}). The log determining in \eqref{eq:log-ll} can be efficiently computed by $\log |\K_{\Zcal\Zcal}| = \sum\nolimits_{j} (N/N_j)\log|\K_j|$ where $N = \prod_j N_j$. 

\begin{algorithm}[t]
	\small 
	\caption{EP-EM($\Dcal$, $\Fcal$, $T$, $\xi$, $\tau_2$)}          
	\label{alg:ep-em}                           
	\begin{algorithmic}[1]                    % enter the algorithmic environment
		\STATE Learn a GP model from $\Dcal$ to obtain an initial estimate of $\boldeta$ and the kernel parameters $\btheta$. Obtain $\tau_1$ from cross-validation. \zhec{check with Da about $\tau_2$}
		\REPEAT
		\STATE E-step: Fix $\boldeta$ and $\btheta$, run EP until convergence to estimate   $q(\s, \w) \approx p(\s,  \w|\Dcal)$ in \eqref{eq:qws}, using the updates XXX in Sec XXX of the Appendix.  
		\STATE M-step: Fix $q(\s, \w)$, maximize \eqref{eq:log-ll-2} with ADAM to update $\boldeta$ and $\btheta$.  
		\UNTIL {$T$ iterations are done or the relative change of $\boldeta$ is less than $\xi$}
		\RETURN $q(\s, \w)$, $\boldeta$ and $\btheta$. 
	\end{algorithmic}\label{algo:ep-em}
	%\vspace{-0.05in}
\end{algorithm}

To further save the cost and to decouple the strong dependency between $\Ucal$ and the kernel parameters, we use the whitening method [] to reparameterize $\Ucal$, 
\begin{align}
	\vec(\Ucal) = \L_{\Zcal\Zcal} \cdot \vec(\boldeta), \;\;\; \K_{\Zcal\Zcal} = \L_{\Zcal\Zcal}\L_{\Zcal\Zcal}^\top, \;\;\; \boldeta \sim \N(\boldeta|\0, \I).
\end{align}
To obtain the Cholesky factors $\Lcal_{\Zcal\Zcal}$, we can first perform Cholesky decomposition at each input dimension, $\K_j = \L_j \L_j^\top$. We then have $\K_{\Zcal\Zcal} = \L_1 \L_1^\top \kron \ldots \kron \L_{m+1}\L_{m+1}^\top = \left(\L_1 \kron \ldots \kron \L_{m+1}\right)\left(\L_1 \kron \ldots \kron \L_{m+1}\right)^\top$
and hence $\L_{\Zcal\Zcal} = \L_1 \kron \ldots \kron \L_{m+1}$ and $\vec(\Ucal)  =\left( \L_1 \kron \ldots \kron \L_{m+1}\right) \vec(\boldeta)$.
Again, according to the definition of the Tucker operator, we can efficiently compute $\Ucal$ from $\boldeta$ with tensor-matrix products, 
\begin{align}
	\Ucal = \boldeta \times_1 \L_1 \times_2 \ldots \times_{m+1} \L_{m+1}. 
\end{align}
\cmt{With $\Ucal$, we then compute derivative values on $\Zcal$ and function values at the training inputs.} We therefore maximize the expected log likelihood w.r.t to $\boldeta$ and the kernel parameters, 
\begin{align}
	\widehat{\Lcal} =  - \frac{1}{2}\vec(\boldeta)^\top \vec(\boldeta) - \frac{1}{2}\tau_1 \| \y - \f\|^2   - \frac{1}{2}\tau_2\EE_q\left[ \|\h - \bPhi \w\right\|^2] + \text{const}. \label{eq:log-ll-2}
\end{align}
Note that the first term now corresponds to the log prior of $\boldeta$, which is the standard Gaussian and does not include $\K_{\Zcal\Zcal}$ anymore. Our model estimation is summarized in Algorithm \ref{alg:ep-em}. 

\cmt{
Specifically, to compute each $f_j$ in \eqref{eq:kint-1}, we have 
\begin{align}
	f_n &= \left(\kappa(x_{n,1}, \z_1) \kron \ldots \kron \kappa(x_{n,{m+1}},\z_{m+1})\right) (\K_1^{-1} \kron \ldots \kron \K_{m+1}^{-1})\vec(\Ucal) \notag \\
	&= \left(\kappa(x_{n,1}, \z_1) \K_1^{-1} \kron \ldots \kron \kappa(x_{n,m+1},\z_{m+1})\K_{m+1}^{-1}\right) \vec(\Ucal) \notag \\
	&= \Ucal \times_1 \kappa(x_{n,1}, \z_1) \K_1^{-1} \times_2 \ldots \times_{m+1} \kappa(x_{n,m+1},\z_{m+1})\K_{m+1}^{-1}
\end{align}
where $\times_j$ is tensor-matrix product at mode $j$. Therefore, we can compute $\kappa(x_{n,j}, \z_j) \K_j^{-1}$ at each dimension $j$, and then use the tensor-matrix product to compute the $f_n$. 
}


\cmt{
According to the properties of the Kronecker product, we have 
\begin{align}
	\log |\K_{\Zcal\Zcal}| &= \sum\nolimits_{j} (N/N_j)\log|\K_j|, \notag \\
	\K_{\Zcal\Zcal}^{-1} \vec(\Ucal) &= 
\end{align}
where $N = \prod_j N_j$
}

%We now present the model estimation algorithm. Given the training data $\Dcal$ and collocation points $\Zcal$, we aim to estimate the posterior distribution of $\u$, $\g$, the coefficients $\w$,  and the kernel parameters. This is challenging, because the HS density in \eqref{eq:hs} does not have a closed-form. In addition, when the number of collocation points is large, the covariance matrix in the multivariate Gaussian prior \eqref{eq:gp-joint} is prohibitively expensive to compute. To address these issues, we introduce  auxiliary variables to represent the HS prior,  use the variational inducing-point method to evade computing the huge covariance matrix, and  develop an efficient structural variational inference algorithm.% with the re-parameterization trick. 

\cmt{
Specifically, we first introduce auxiliary variables to sample each $\lambda_j^2$ and $s^2$ in the HS prior \eqref{eq:hs} via a nested inverse Gamma (NIG) structure~\citep{wand2011mean}, which is equivalent to the half-Cauchy prior of $\lambda_j$ and $s$, 
\begin{align}
	\lambda_j^2 | v_j  \sim \text{IG}(\frac{1}{2}, \frac{1}{v_j}), \;\; v_j \sim \text{IG}( \frac{1}{2}, \frac{1}{a_0}), \notag \\
	s^2 | \alpha \sim \text{IG}(\frac{1}{2}, \frac{1}{\alpha}), \;\; \alpha \sim \text{IG}(\frac{1}{2}, \frac{1}{a_1}), \label{eq:nig}
\end{align}
where $\text{IG}(x|\beta_0,\beta_1) = \frac{\beta_1^{\beta_0}}{\Gamma(\beta_0)}x^{-\beta_0 - 1}\exp(-\frac{\beta_1}{x})$ and $\Gamma(\cdot)$ is the Gamma function.
Similar to the whitening method often used in GP inference~\citep{murray2010slice}, we represent $w_j = \lambda_j s \xi_j$ according to \eqref{eq:hs} where $\xi_j \sim \N(0, 1)$, so as to reduce the prior dependency and ease the posterior inference. 
 Therefore, the joint distribution of our model with the auxiliary variables is 
\begin{align}
	&p(\u, \g, s^2, \alpha, \{\lambda_j^2, v_j\}_{j=1}^M) =  \N\left([\u; \g]|\0, \bSigma\right) \text{NIG}(s^2, \alpha|a_1)  \notag \\
	& \cdot \prod\nolimits_{j=1}^M \text{NIG}(\lambda_j^2, v_j|a_0) \N(\xi_j|0, 1) \cdot \N(\y|\f, \sigma_0^2\I) \N\left(\wy|\brho - \sum\nolimits_{j} w_j \bphi_j, \sigma_1^2\I\right), \label{eq:joint-2}
\end{align}
where $\text{NIG}(\eta, \gamma|a) = \text{IG}(\eta|\frac{1}{2}, \frac{1}{\gamma})\text{IG}(\gamma|\frac{1}{2}, \frac{1}{a}) $.  

We then consider the variational inference approach for posterior estimation~\citep{wainwright2008graphical}. Given a variational posterior $q(\Theta)$, we construct a variational model evidence lower bound (ELBO), 
\begin{align}
	\Lcal = \EE_{q}\left[\frac{p(\u, \g, s^2, \alpha, \{\lambda_j^2, v_j\}_{j=1}^M)}{q(\Theta)}\right] \label{eq:elbo}
\end{align}
where $\Theta = \{\u, \g, s^2, \alpha, \{\lambda_j^2, v_j\}\}$ includes all the latent random variables. We maximize $\Lcal$ to estimate $q(\Theta)$. For efficient computation, we design that $q(\Theta)$ is factorized across the variables.  Specifically, similar to \citep{ghosh2019model}, we introduce a log normal posterior (LN) for $s^2$ to ensure  positivity, which is also convenient to apply the reparameterization trick~\citep{kingma2013auto} for efficient stochastic optimization. Since  each $w_j = s \lambda_j \xi_j$,  the local scales $\{\lambda_j\}$ and local Gaussian noises $\{\xi_j\}$  can be highly correlated in the true posterior. To capture their dependency, we introduce a matrix Gaussian variational posterior for $\A =[\blambda, \bxi]$ where $\blambda = [\log(\lambda_1^2); \ldots; \log(\lambda_M^2)]$ and $\bxi = [\xi_1; \ldots; \xi_M]$, 
\begin{align}
	q(\A) = \mathcal{MN}(\A | \bar{\A}, \bOmega_1, \bOmega_2) = \N(\vec(\A)| \vec(\bar{\A}), \bOmega_1 \kron \bOmega_2),
\end{align}
where $\bar{\A}$ is the mean, $\bOmega_1$ is the $M\times M$ row covariance matrix, and $\bOmega_2$ is the $2 \times 2$  column covariance matrix. To ensure the positive definiteness, we further parameterize $\bOmega_1 = \L_1 \L_1^\top$ and $\bOmega_2 = \L_2 \L_2^\top$ where $\L_1$ and $\L_2$ are lower-triangular matrices. In this way, not only can we capture the full posterior correlations in $\A$, we also save the parameters and do not need to estimate the $2M \times 2M$ entire covariance matrix.  The matrix Gaussian is also convenient for us to use the reparameterization trick.

A severe computational challenge arises when the number of collocation points $G$ is large ---  the covariance matrix of the multivariate Gaussian prior $p(\u, \g) =  \N\left([\u; \g]|\0, \bSigma\right)$ in \eqref{eq:joint-2} is huge and prohibitively costly to calculate. To address this issue, we use an idea similar to the variational inducing-point method~\citep{hensman2013gaussian}. We observe that the joint prior can be decomposed as $p(\u, \g) = \N(\u|\0, \bSigma_{uu}) p(\g|\u)$, where $p(\g|\u)$ is a giant conditional Gaussian distribution. We then introduce the variational posterior for $\u$ and $\g$ as %$q(\u, \g) = q(\u) p(\g|\u)$, 
\begin{align}
	q(\u, \g) = q(\u) p(\g|\u), 
\end{align}
where $q(\u) = \N(\u|\bmu_u, \L_u\L_u^\top)$ is a Gaussian distribution, and $\L_u$ is a lower triangular matrix. Accordingly, when we compute the log fraction inside the ELBO in \eqref{eq:elbo}, the conditional Gaussian will cancel out, 
\begin{align}
	&\Lcal = \EE_{q}\left[\frac{\N(\u|\0, \bSigma_{uu}) \bcancel{p(\g|\u)}  p(\wy|\bPhi, \w)\cdot \text{Others}}{q(\u) \bcancel{p(\g|\u)} q(\text{Others})}\right] \notag \\
	&= -\text{KL}(q(\u) \| \N(\u|\0, \bSigma_{uu})) + \sum\nolimits_{n=1}^G \EE_{q}\left[\log  \N(\widehat{y}_n | \rho_n - \sum\nolimits_j w_j \phi_{jn}, \sigma_1^2) \right] + \text{Others}, 
\end{align} 
where $\text{KL}(\cdot \| \cdot)$ is the Kullback-Leibler divergence, and $\bSigma_{uu} = \L_u \L_u^\top$. Since the virtual likelihood is a diagonal Gaussian (see \eqref{eq:vll}), the ELBO is additive over each collocation point. That means, we no longer need to compute the giant full conditional Gaussian $p(\g|\u)$. Instead, we compute the KL divergence regarding $\u$ only (based on the small training dataset), and  the conditional distribution of the elements of $\g$ associated with each individual collocation point, which is a small subset, and hence much cheaper to compute.  The additive form over the collocation points further enables us to  sample a mini-batch of collocation points each time, and use the reparameterization trick to update the posterior parameters with stochastic optimization.  %We sample a mini-batch of collocation points each time, and use the reparameterization trick to update the posterior parameters. 

Finally, our variational posterior has the following form, 
\begin{align}
	q(\Theta) =  \LN(s^2|\mu_s, \tau_s) q(\alpha) \prod\nolimits_{j} q(v_j) \cdot \mathcal{MN}(\A|\bar{\A}, \L_1\L_1^\top, \L_2\L_2^\top)q(\u) p(\g|\u). \notag 
\end{align}
We substitute it into \eqref{eq:elbo} to obtain the actual ELBO, and then apply stochastic mini-batch  optimization.  We use the mean-field variational update~\citep{bishop2006pattern} for $q(\alpha)$ and each $q(v_j)$, which gives the optimal form, \ie inverse Gamma, and thereby we do not need to design an additional posterior approximation term.  Each step, we first update the posterior of the other variables via stochastic gradient ascent, and then update $q(\alpha)$ and each $q(v_j)$ accordingly.   
}


==> related-fang.tex <==
%\vspace{-0.05in}
\section{Related Work}
%\vspace{-0.1in}
%There is a large body of related work. Due to the space limit, we briefly discuss the most related lines of work. 
%\cmt{PINNs have shown promise as a computationally efficient alternative to expensive mesh-based numerical methods such as finite elements and finite volumes~\citep{reddy2019introduction}.\cmt{~\citep{long2018pde, han2018solving}.}}\cmt{PINNs (typically) work by \textit{softly} constraining neural networks to abide by physical constraints given well-studied governing equations --- a strategy that is beneficial particularly in the small data regime~\citep{rackauckas2020universal, lu2021deepxde, weinan2017deep, raissi2019physics, hennigh2021nvidia}. }
Although the PINN has many success stories, \eg~\citep{raissi2020hidden, chen2020physics, jin2021nsfnets, sirignano2018dgm, zhu2019physics, geneva2020modeling, sahli2020physics}, the training is known to be challenging, which is partly due to that applying differential operators over the NN can complicate the loss landscape~\citep{krishnapriyan2021characterizing}. Recent works have analyzed common failure modes of PINNs which include modeling problems exhibiting high-frequency, multi-scale, chaotic, or turbulent behaviors~\citep{wang2020and, wang2020eigenvector, wang2020understanding, wang2022respecting}, or when the governing PDEs are stiff~\citep{krishnapriyan2021characterizing, mojgani2022lagrangian}. 
One class of approaches to mitigate the training challenge is to set different weights for the boundary and residual loss terms. For example, \citet{wight2020solving} suggested to set a large weight for the boundary loss to prevent the dominance of the residual loss.  \citet{wang2020understanding} proposed a dynamic weighting scheme based on the gradient statistics of the loss terms. \citet{wang2020and} developed an adaptive weighting approach based on the eigen-values of NTK. \citet{liu2021dual} employed a mini-max optimization and update the loss weights via stochastic ascent. \citet{mcclenny2020self} used a multiplicative soft attention mask to dynamically re-weight the loss term on each data point and collocation point.
Another strategy is to modify the NN architecture so as to exactly satisfy the boundary conditions, \eg ~\citep{lu2021physics,lyu2020enforcing, lagaris1998artificial}.  However, these methods are restricted to particular types of boundary conditions, and are less flexible than the original PINN framework. \citet{tancik2020fourier,wang2021eigenvector} used Gaussian distributions to construct random Fourier features to improve the learning of the high-frequency and multi-scale information. The number of Gaussian variances and their scales are critical to the success of these methods. But these hyperparameters are quite difficult to choose. 

Earlier works \citep{graepel2003solving,raissi2017machine} have used GP for solving linear PDEs with noisy measurement of source terms. In \citep{wang2021bayesian}, the rationale and guarantees of using GP as a prior for PDE solutions are discussed. The recent work  \citep{chen2021solving} develops a general approach for solving both linear and nonlinear PDEs. \citet{pmlr-v162-long22a} proposed a GP framework to integrate various differential equations. Due to the space limit, we put more discussions on related works that solve PDEs with GP and kernel methods in Section \ref{sect:related-GP-PDE} of Appendix. 

%GP/GP solvers; Neural operators 
%Our work develops a  solver based on GP plus the spectral mixture kernel for solving high-frequency and multi-scale problems.  

%Another recent line of research is to predict the PDE solutions given the source function (or initial conditions). These methods essentially are learning a function-to-function mapping. The typical examples include Fourier neural operators (FNO)~\citep{li2020fourier} and deep operator net (DeepONet)~\citep{lu2019deeponet,lu2021learning}. Different from PINNs and other  machine learning based solvers, these methods do not attempt to solve a particular PDE. Their learning even does not need to know the PDE form. Instead, they require  instances of the source functions (or initial conditions) and the solutions of the corresponding PDEs for training. Then they can predict a new PDE's solution with a different source. By contrast, the solvers do not need solution data and only focus on solving one particular equation. 


\cmt{
uses  kernel methods/GPs to estimate the solution function and spatially-varying coefficients in PDE discovery. GPs/kernel methods have been applied for solving differential equations for a long time. For example, \citet{graepel2003solving,raissi2017machine} used GPs to solve linear PDEs with the noisy source term measurements. The recent work \citep{chen2021solving}  developed a general kernel method to solve both linear and nonlinear PDEs. But all these methods assume the equations are given and cannot discover the equations from data.  GPs have also been used to model the equation components or incorporate the equations for better training. For example, \citet{heinonen2018learning} used GPs to model the dynamics of unknown ODEs.  \citet{alvarez2009latent} proposed latent force models to incorporate incomplete equations into GP training. Other examples include ~\citep{barber2014gaussian,macdonald2015controversy, heinonen2018learning,lorenzi2018constraining,wenk2019fast,wenk2020odin,pan2020physics}. 
The GP community has realized the computational advantage of the Kronecker product for a long time~\citep{saatcci2012scalable}, and there has been works in leveraging the Kronecker product properties to improve the training speed and scalability, such as high-dimension output regression~\citep{zhe2019scalable} and sparse approximation based on inducing points~\citep{wilson2015kernel,izmailov2018scalable}.  
However, in many typical GP applications, the function values are not observed at a grid and the Kronecker product structure has a limited usage. By contrast, for PDE solution learning, it is natural to estimate the function values on a mesh (which is consistent with the practice of traditional numerical methods), which opens the possibility of using Kronecker products for efficient computation. To our knowledge, our work is first to realize this point and use the product kernels to derive the Kronecker  product structure in the kernel matrix and to enable efficient, scalable function estimation, without the need for low-rank approximations. 
}
